Tailoring 3D Speckle Statistics

We experimentally generate three-dimensional speckles with customized intensity statistics. By modulating the phase front of a laser beam, far-field speckle patterns maintain the designed intensity probability density function while evolving to different spatial patterns upon axial propagation. We also create speckles with distinct intensity statistics at multiple designated planes. These results open many new possibilities, such as designing volumetric speckle statistics for three-dimensional imaging, sensing, trapping, and manipulation.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
